Random Permutations -- A geometric point of view

We look at geometric limits of large random non-uniform permutations. We mainly consider two theories for limits of permutations: permuton limits, introduced by Hoppen, Kohayakawa, Moreira, Rath, and Sampaio to define a notion of scaling limits for permutations; and Benjamini-Schramm limits, introduced by the author to define a notion of local limits for permutations. The models of random permutations that we consider are mainly constrained models, that is, uniform permutations belonging to a given subset of the set of all permutations. We often identify this subset using pattern-avoidance, focusing on: permutations avoiding a pattern of length three, substitution-closed classes, (almost) square permutations, permutation families encoded by generating trees, and Baxter permutations. We explore some universal phenomena for the models mentioned above. For Benjamini-Schramm limits we explore a concentration phenomenon for the limiting objects. For permuton limits we deepen the study of some known universal permutons, called biased Brownian separable permutons, and we introduce some new ones, called Baxter permuton and skew Brownian permutons. In addition, for (almost) square permutations, we investigate the occurrence of a phase transition for the limiting permutons. On the way, we establish various combinatorial results both for permutations and other related objects. Among others, we give a complete description of the feasible region for consecutive patterns as the cycle polytope of a specific graph; and we find new bijections relating Baxter permutations, bipolar orientations, walks in cones, and a new family of discrete objects called coalescent-walk processes.

==> frontmatter/abbreviations.tex <==
%% will only print what is used ... useful.
%% also acronyms are clickable, which is awesome

\chapter*{List of Abbreviations}
\markboth{List of Abbreviations}{List of Abbreviations}


               
%\begin{acronym}\itemsep-20pt\parsep-20pt %% if you remove these spacing params this list becomes huge!
%\acro{CDMA}{Code Division Multiple Access}
%\acro{GSM}{Global System for Mobile communication}
%\acro{NAD+}[NAD\textsuperscript{+}]{Nicotinamide Adenine Dinucleotide}
%\acro{NUA}{Not Used Acronym}
%\acro{TDMA}{Time Division Multiple Access}
%\acro{UA}{Used Acronym}
%\acro{lox}[\ensuremath{LOX}]{Liquid Oxygen}
%\acro{lh2}[\ensuremath{LH_2}]{Liquid Hydrogen}
%\acro{IC}{Integrated Circuit}
%\acro{BUT}{Block Under Test}
%\acrodefplural{BUT}{Blocks Under Test}    
%\end{acronym}




==> frontmatter/originality.tex <==
\begin{originality}
\end{originality}
